Galactic Dynamos

Spiral galaxies, including the Milky Way, have large-scale magnetic fields with significant energy densities. The dominant theory attributes these magnetic fields to a large-scale dynamo. We review the current status of dynamo theory and discuss various numerical simulations designed to explain either particular aspects of the problem or to reproduce galactic magnetic fields globally. Our main conclusions can be summarized as follows. Idealized direct numerical simulations produce mean magnetic fields, whose saturation energy density tends to decline with increasing magnetic Reynolds number. This is still an unsolved problem. Large-scale galactic magnetic fields of microgauss strengths can probably only be explained if helical magnetic fields of small or moderate length scales can rapidly be ejected or destroyed. Small-scale dynamos are important throughout a galaxy's life, and probably provide strong seed fields at early stages. The circumgalactic medium (CGM) may play an important role in driving dynamo action at small and large length scales. These interactions between the galactic disk and the CGM may provide important insights into our understanding of galactic dynamos. We expect future research in galactic dynamos to focus on the cosmological history of galaxies and the interaction with the CGM as means of replacing the idealized boundary conditions used in earlier work.

==> figure_comments_04_23.tex <==
Figure 1: No comment/change.

Figure 2: 
GM: Can descriptive title labels (with units if applicable) be added to these colorscale bars?
AB: we have now added the symbol with units in the second panel.

Figure 3: 
GM: Part labels have been added—OK?
Please review label placement in part a and conrm if correct.
Can a key be added to part c with the colors described in the caption?
- We Re-did the figure and added a key. 

Figure 4:
GM: A key has been added to the Figure.
Please review and confirm if correct.
- Keys are correct.
GM: Please review these symbols and confirm if correct.
- Symbols are correct.

Figure 5:
GM: Please review symbols
and confirm if correct.
- Symbols are correct.

Figure 6:
GM: Please review symbols
and confirm if correct.
- Symbols are correct.
GM: (about the caption) There doesn’t appear to be a gray line in this figure.
Please advise.
- Indeed, the caption refers to an older version of the figure. It should be replaced with "dotted lines show the mean vertical flow."

Figure 7:
-The supplied file for this figure was low resolution and has been redrawn.
Most of the labels have been retyped. Please review carefully and confirm if correct.
- Correct. 
GM: (about the caption) Can this section be clarified?
Is “a few strength” intended to mean weakness,
lower magnification, or something else?
- It seems to be a typo, meant to be "permissible field strength"

Figure 8: 
GM: Can a descriptive title label (including units, if applicable)
be added to the colorscale bar here?
- The title label is "Rotation Measure [rad/m$^2$]". It would probably be easier for you to add it, since she has to re-type all the labels anyway.

Figure 9:
All labels in this figure have been retyped.
Please review and confirm if okay.
Part labels have been added—OK?
- It all looks fine.

Figure 10:
GM: All labels in this figure have been retyped.
Please review and confirm if okay.
Part labels have been added—OK?
Color has been added to the graphs for visual interest—OK?
Please review and confirm if correct.
- Seems fine, also with the color.

Figure 11:
GM: All labels in this figure have been retyped. Please review and confirm if correct.
- Labels are correct.
GM: Please add a section for abbreviations and define RM.
AB: RM is actually defined on page 4 in the text box. There are otherwise no abbreviations in the paper.

Figure 12:
GM: All labels in this figure have been retyped.
Color has been added to part b for visual interest—OK?
Please review and confirm if correct.
- Correct.

Figure 13:
GM: All labels in this figure have been retyped. Please review and confirm if correct.
- Correct

Figure 14:
GM: The layout of this figure has been changed to better fit the page, with the colorscale bars
moved below each part. Please double-check that the parts and labels are set as desired.
Please review carefully and confirm if correct.
- Correct.

Figure 15:
No comment/change.

